Value Functions for Depth-Limited Solving in Zero-Sum Imperfect-Information Games

We provide a formal definition of depth-limited games together with an accessible and rigorous explanation of the underlying concepts, both of which were previously missing in imperfect-information games. The definition works for an arbitrary extensive-form game and is not tied to any specific game-solving algorithm. Moreover, this framework unifies and significantly extends three approaches to depth-limited solving that previously existed in extensive-form games and multiagent reinforcement learning but were not known to be compatible. A key ingredient of these depth-limited games are value functions. Focusing on two-player zero-sum imperfect-information games, we show how to obtain optimal value functions and prove that public information provides both necessary and sufficient context for computing them. We provide a domain-independent encoding of the domains that allows for approximating value functions even by simple feed-forward neural networks, which are then able to generalize to unseen parts of the game. We use the resulting value network to implement a depth-limited version of counterfactual regret minimization. In three distinct domains, we show that the algorithm's exploitability is roughly linearly dependent on the value network's quality and that it is not difficult to train a value network with which depth-limited CFR's performance is as good as that of CFR with access to the full game.

==> contribution.tex <==
\paragraph{Contribution}
\edit{We provide both theoretical and empirical contributions.
(1) We provide an accessible description of prerequisites of depth-limited solving in arbitrary imperfect-information domains beyond poker, many of which were previously insufficiently formal or general and have not been written down in a single work (Section~\ref{sec:background:values}).
The key statements of this section are the characterization and properties of value functions (Lemma~\ref{lem:hist-value:characterization} and Theorems~\ref{thm:infoset-v-characterization} and \ref{thm:infoset-cfv-properties}).
With a few explicitly listed exceptions, the results of this section are well-known or simple;
    the main contribution of this section lies in formalizing and organizing the content in one place.
In contrast, the remainder of the formal results (Section~\ref{sec:theory}) are novel unless stated otherwise.}

\edit{(2) Formalizing the prerequisites allows us to provide a domain- and algorithm- independent definition of a depth-limited game,  the complementary notion of a value function, and a number of relevant concepts (Section~\ref{sec:DL_games}).
This enables us to relate several previously seemingly-different results on depth-limited solving (Section~\ref{sec:noam} and Section~\ref{sec:fog}).
(2) We introduce several notions of optimality of value functions with the main result being formal proofs that lead to optimal solutions of depth-limited solving  (Theorem~\ref{thm:reach_opt_preserve_NE} and Theorem~\ref{thm:portfolio-game}). In addition, we find a compact representation for value functions in imperfect-information games and we identify and prove the minimal context over which they need to be defined which were only implicitly  present in  the  proofs or explained in domain-specific terms
in the previous work (Theorem~\ref{thm:wholeRangeDep}). On top of that, we provide an analysis of their uniqueness and convexity. (3) We show that a general domain-independent neural network architecture can be used to approximate the value function of several distinctly different domains and produce near-optimal strategies when used in depth-limited solving. We show how the value network's error is related to the quality of the produced strategy (Figure~\ref{fig:expl_vs_error2}) and explore the value network's generalization abilities (Figure~\ref{fig:pubstatecrossval_main2}, \ref{app:sec:loss}).} 
% (3) In Section~\ref{sec:sub:encoding}, we show how a novel formalism, factored-observation stochastic games, can be used to encode the information necessary to train a neural network to approximate the value function in arbitrary imperfect-information games.
% and perform a qualitative comparison of \DLCFR to a state-of-the-art algorithm (Figure~\ref{fig:heatmap_main2}). 
